MMFactory: A Universal Solution Search Engine for Vision-Language Tasks

With advances in foundational and vision-language models, and effective fine-tuning techniques, a large number of both general and special-purpose models have been developed for a variety of visual tasks. Despite the flexibility and accessibility of these models, no single model is able to handle all tasks and/or applications that may be envisioned by potential users. Recent approaches, such as visual programming and multimodal LLMs with integrated tools aim to tackle complex visual tasks, by way of program synthesis. However, such approaches overlook user constraints (e.g., performance / computational needs), produce test-time sample-specific solutions that are difficult to deploy, and, sometimes, require low-level instructions that maybe beyond the abilities of a naive user. To address these limitations, we introduce MMFactory, a universal framework that includes model and metrics routing components, acting like a solution search engine across various available models. Based on a task description and few sample input-output pairs and (optionally) resource and/or performance constraints, MMFactory can suggest a diverse pool of programmatic solutions by instantiating and combining visio-lingual tools from its model repository. In addition to synthesizing these solutions, MMFactory also proposes metrics and benchmarks performance / resource characteristics, allowing users to pick a solution that meets their unique design constraints. From the technical perspective, we also introduced a committee-based solution proposer that leverages multi-agent LLM conversation to generate executable, diverse, universal, and robust solutions for the user. Experimental results show that MMFactory outperforms existing methods by delivering state-of-the-art solutions tailored to user problem specifications. Project page is available at https://davidhalladay.github.io/mmfactory_demo.

==> figures/exp_iteranalysis_tikz.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=10cm, height=8cm,
        xlabel={Iteration},
        ylabel={Accuracy},
        ymin=0, ymax=0.8,
        xmin=1, xmax=6,
        xtick={1, 2, 3, 4, 5, 6},
        xticklabels={1\textsuperscript{st} iter, 2\textsuperscript{ed} iter, 3\textsuperscript{rd} iter, 4\textsuperscript{th} iter, 5\textsuperscript{th} iter, 6\textsuperscript{th} iter},
        ytick={0, 0.2, 0.4, 0.6, 0.8},
        legend style={at={(1.05,1)}, anchor=north west},
        legend columns=2,
        grid=major,
    ]

    % Data for each run with sample points
    \addplot[mark=*, color=cyan] coordinates {(1,0.2) (2,0.6) (3,0.5) (4,0.7) (5,0.6) (6,0.4)};
    \addlegendentry{run 1}

    \addplot[mark=*, color=blue] coordinates {(1,0.3) (2,0.5) (3,0.7) (4,0.6) (5,0.5) (6,0.3)};
    \addlegendentry{run 2}

    \addplot[mark=*, color=red] coordinates {(1,0.1) (2,0.7) (3,0.6) (4,0.5) (5,0.4) (6,0.2)};
    \addlegendentry{run 3}

    \addplot[mark=*, color=green] coordinates {(1,0.4) (2,0.6) (3,0.5) (4,0.7) (5,0.3) (6,0.4)};
    \addlegendentry{run 4}

    \addplot[mark=*, color=purple] coordinates {(1,0.3) (2,0.8) (3,0.6) (4,0.4) (5,0.5) (6,0.3)};
    \addlegendentry{run 5}

    \addplot[mark=*, color=pink] coordinates {(1,0.2) (2,0.5) (3,0.4) (4,0.6) (5,0.6) (6,0.3)};
    \addlegendentry{run 6}

    \addplot[mark=*, color=orange] coordinates {(1,0.1) (2,0.4) (3,0.5) (4,0.5) (5,0.4) (6,0.2)};
    \addlegendentry{run 7}

    \addplot[mark=*, color=yellow] coordinates {(1,0.2) (2,0.3) (3,0.4) (4,0.6) (5,0.5) (6,0.3)};
    \addlegendentry{run 8}

    \addplot[mark=*, color=gray] coordinates {(1,0.3) (2,0.7) (3,0.6) (4,0.5) (5,0.4) (6,0.2)};
    \addlegendentry{run 9}

    \addplot[mark=*, color=lime] coordinates {(1,0.4) (2,0.6) (3,0.5) (4,0.7) (5,0.5) (6,0.3)};
    \addlegendentry{run 10}

    % Mark points with black cross marks
    \addplot[only marks, mark=x, mark size=4pt, color=black] coordinates {(2,0.6) (3,0.7) (4,0.7) (5,0.6)};
    
    \end{axis}
\end{tikzpicture}

==> figures/exp_timecost.tex <==

% \begin{figure}[t]
%   \centering
%   \includegraphics[page=18, trim={180 60 130 40}, clip, width=\columnwidth]{figures/sources/MMFactory_figures.pdf}
%   \vspace{-3mm}
%   \caption{\textbf{Time cost analysis for API calling}. }
%   \label{exp:time_cost}
%   \vspace{-4mm}
% \end{figure}

% \begin{table}[]
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{l|cc|cc}
% \toprule
% \multicolumn{1}{c|}{\multirow{2}{*}{Model}} & \multicolumn{2}{c|}{Execution cost (sec)} & \multicolumn{2}{c}{Routing cost (sec)} \\ \cline{2-5} 
% \multicolumn{1}{c|}{} & Mean & Variance & Mean & Variance \\ \hline
% sketchpad & 19.96 & 43.86 & 18.20 &	30.90 \\ \hline
% Ours & 9.74 & 29.43 & $\approx$ 0.00 & $\approx$ 0.00 \\
% \bottomrule
% \end{tabular}}
% \caption{\textbf{API calling cost analysis}}
% \vspace{-0.25in}
% \end{table}

% \begin{figure}[t]
%   \centering
%   % First row: Figure
%   \begin{minipage}{\columnwidth}
%     \centering
%     \includegraphics[page=18, trim={180 35 130 40}, clip, width=\columnwidth]{figures/sources/MMFactory_figures.pdf}
%     \vspace{-3mm}
%     \caption{\textbf{Time cost analysis for API calling}.}
%     \label{exp:time_cost}
%   \end{minipage}
%   \vspace{5mm} % Adjust spacing between figure and table as needed

%   % Second row: Table
%   \begin{minipage}{\columnwidth}
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l|cc|cc}
%       \toprule
%       \multicolumn{1}{c|}{\multirow{2}{*}{Model}} & \multicolumn{2}{c|}{Execution cost (sec)} & \multicolumn{2}{c}{Routing cost (sec)} \\ \cline{2-5} 
%       \multicolumn{1}{c|}{} & Mean & Variance & Mean & Variance \\ \hline
%       sketchpad & 19.96 & 43.86 & 18.20 & 30.90 \\ \hline
%       Ours & 9.74 & 29.43 & $\approx$ 0.00 & $\approx$ 0.00 \\
%       \bottomrule
%     \end{tabular}}
%     \caption{API calling cost analysis}
%   \end{minipage}
%   \vspace{-4mm}
% \end{figure}
